Fast and Feature-Complete Differentiable Physics for Articulated Rigid Bodies with Contact

We present a fast and feature-complete differentiable physics engine, Nimble (nimblephysics.org), that supports Lagrangian dynamics and hard contact constraints for articulated rigid body simulation. Our differentiable physics engine offers a complete set of features that are typically only available in non-differentiable physics simulators commonly used by robotics applications. We solve contact constraints precisely using linear complementarity problems (LCPs). We present efficient and novel analytical gradients through the LCP formulation of inelastic contact that exploit the sparsity of the LCP solution. We support complex contact geometry, and gradients approximating continuous-time elastic collision. We also introduce a novel method to compute complementarity-aware gradients that help downstream optimization tasks avoid stalling in saddle points. We show that an implementation of this combination in an existing physics engine (DART) is capable of a 87x single-core speedup over finite-differencing in computing analytical Jacobians for a single timestep, while preserving all the expressiveness of original DART.

==> introduction.tex <==
\section{Introduction}
\label{intro}

%With the rise of deep learning, researchers in robotics have turned to deep reinforcement learning as a standard approach for solving challenging control tasks, in part because standard physics engines are non-differentiable~\cite{bullet,todorov2012mujoco,dart,drake}. 

With the rise of deep learning, interest in differentiable physics engines has grown for applications from optimal control to policy learning to parameter estimation. While many differentiable physics engines have been proposed in recent years to the robotics community, none so far has replaced commonly used non-differentiable physics engines \cite{bullet,todorov2012mujoco,dart,drake}, which offer a complete set of features for forward simulating complex articulated rigid body systems.

Physics engines for robotic applications have a set of desired requirements including representing states in the generalized (reduced) coordinates and solving constraint satisfaction problems for contact and other mechanical constraints. Existing \emph{feature-complete} physics engines with such capabilities have been validated and stress-tested by a large number of users across multiple communities \cite{gazebo,openAI,opensim}. An ideal differentiable physics engine should neither compromise these requirements nor reinvent the forward simulation process in exchange for differentiability. It should also support the complete feature set of an existing physics engine, including various joint types, different actuation mechanisms, and complex contact geometry. Above all, it must be computationally efficient such that real-time control and identification problems on complex robotic platforms can be enabled.

In this paper, we take an existing engine commonly used in robotics and graphics communities and make it differentiable. Our engine supports all features available to the forward simulation process, meaning existing code and applications will remain compatible while also enjoying new capabilities enabled by differentiability. We extend a fast, stable, industry-standard physics engine, DART, to compute analytical gradients in the face of hard contact constraints. By introducing an efficient method for LCP differentiation that exploits sparsity, novel contact geometry algorithms, and an efficient continuous-time approximation for elastic collisions, our engine is able to compute gradients with hard contact constraints up to 45 times faster than finite differencing methods, depending on the size of the dynamic system. Our relative speedup over finite differencing grows as the system complexity grows, so on Boston Dynamics' Atlas robot (the most complex robot we test against, pictured above), we achieve our best relative performance with a 45x speedup.

\begin{figure}
\centering
\includegraphics[width=8.2cm]{figures/AtlasYoga2.png}
\vspace{-0.2cm}
\caption{Boston Dynamics' Atlas Robot learning to do yoga, being simulated by our engine. This robot has 34 mesh colliders and 32 degrees of freedom. This freeze frame contains 24 contact points, 12 per foot. Even with all that complexity, we are able to compute the Jacobians of dynamics on this robot \textbf{45x faster} using the analytical methods introduced in this paper than by finite differencing (only \textbf{16ms} vs 737ms for finite differencing).}
\vspace{-0.2cm}
\label{fig:simstep}
\end{figure}


A physics engine that employs hard contact constraints is non-differentiable. While this statement is true, a more interesting question is whether the ``gradient'' we manage to approximate in the face of non-differentiability is of any use for the downstream tasks of interest, such as optimal control or system identification.  The contact handling based on solving an LCP is theoretically differentiable with well-defined gradients, except for a subspace in which a contact state is perfectly balanced between static/sliding or static/breaking. Even in those cases, we show that well-defined subgradients exist and propose a fast method to compute them through the LCP constraints. However, because of the discontinuity of contact states, locally well-defined gradients can be myopic and of little use to the convergence of downstream optimization problems. We also propose a heuristic-based method to compute \emph{complementarity-aware gradients} that are mathematically inconsistent with the forward simulation, but help the optimizer explore discrete contact states and escape saddle points.

We also provide a fast symbolic computation of gradients through collision geometry. We take advantage of the fact that in a discrete-time engine like DART, a small (but non-zero) amount of penetration always exists at the moment a contact point is detected. In order to derive analytical gradients, we assume that an infinitesimally small change to the state will not affect the existence of contact, but will only affect penetration depth. This assumption allows us to compute well-defined gradients and we do so in an efficient and analytically correct way that supports a wide variety of 3D shapes and meshes. However, the discretization of time causes an issue for elastic contact which was initially pointed out by \citet{difftaichi}. We propose an efficient approximation of gradients through continuous-time collisions which is fast enough for complex 3D geometry and dynamic systems in generalized coordinates.

To summarize, our contributions are as follows:
\begin{itemize}
    \item A novel and fast method for local differentiability of LCPs that exploits the sparsity of the LCP solution, which gives us efficient gradients through static and sliding contacts and friction without changing traditional forward-simulation formulations.
    \item A method that manipulates gradient computation to help downstream optimization problems escape saddle points due to discrete contact states. 
    \item Fast geometric analytical gradients through collision detection algorithms which support various types of 3D geometry and meshes.
    \item A novel analytical approximation of continuous-time gradients through elastic contact, which otherwise can lead to errors in discrete-time systems.
    \item An open-source implementation of all of our proposed methods (along with analytical gradients through Featherstone first described in GEAR \cite{kim2012lie}) in a fork of the DART physics engine. We have created Python bindings and a \texttt{pip install} package for ease of use.
\end{itemize}

